Adaptive FE-BE Coupling for Strongly Nonlinear Transmission Problems with Coulomb Friction

We analyze an adaptive finite element/boundary element procedure for scalar elastoplastic interface problems involving friction, where a nonlinear uniformly monotone operator such as the p-Laplacian is coupled to the linear Laplace equation on the exterior domain. The problem is reduced to a boundary/domain variational inequality, a discretized saddle point formulation of which is then solved using the Uzawa algorithm and adaptive mesh refinements based on a gradient recovery scheme. The Galerkin approximations are shown to converge to the unique solution of the variational problem in a suitable product of L^p- and L^2-Sobolev spaces.

==> ex35a90rini.tex <==
21&0.1945908&---&0.1510064&---&1.0265069&0.1895660&0.1471070&22&0.19601 \\
32&0.1602214&-0.461&0.1205155&-0.535&0.8037363&0.1993457&0.1499441&22&0.33202 \\
54&0.1275298&-0.436&0.0918131&-0.520&0.6027735&0.2115717&0.1523177&22&0.64804 \\
93&0.1019990&-0.411&0.0699054&-0.501&0.4422717&0.2306252&0.1580599&22&1.13207 \\
152&0.0821754&-0.440&0.0540462&-0.524&0.3248199&0.2529876&0.1663882&23&2.00013 \\
249&0.0679251&-0.386&0.0449420&-0.374&0.2458318&0.2763072&0.1828161&23&3.35221 \\
400&0.0558447&-0.413&0.0369614&-0.412&0.1902594&0.2935187&0.1942685&23&5.70036 \\
625&0.0439784&-0.535&0.0277857&-0.639&0.1478669&0.2974188&0.1879102&24&9.89662 \\
986&0.0352491&-0.485&0.0217361&-0.539&0.1157059&0.3046439&0.1878565&24&17.4491 \\
1528&0.0279287&-0.531&0.0167409&-0.596&0.0907169&0.3078666&0.1845400&25&31.1619 \\
2322&0.0222760&-0.540&0.0129489&-0.614&0.0713898&0.3120334&0.1813831&25&53.9794 \\
3620&0.0177640&-0.510&0.0102552&-0.525&0.0562611&0.3157421&0.1822787&25&106.743 \\
5544&0.0142059&-0.524&0.0080233&-0.576&0.0444089&0.3198886&0.1806687&25&205.341 \\
8449&0.0112965&-0.544&0.0063426&-0.558&0.0351042&0.3217991&0.1806792&26&422.390 \\
12810&0.0090396&-0.536&0.0050706&-0.538&0.0277777&0.3254265&0.1825421&26&1060.07 \\
19222&0.0072288&-0.551&0.0040370&-0.562&0.0219954&0.3286505&0.1835384&26&2400.17 \\
29006&0.0057984&-0.536&0.0032478&-0.529&0.0174348&0.3325762&0.1862826&27&5459.89 \\
43593&0.0046615&-0.536&0.0026230&-0.524&0.0138332&0.3369792&0.1896163&27&.13E+05 \\


==> ex35h3ini.tex <==
21&0.1945908&---&0.1510064&---&1.0265069&0.1895660&0.1471070&22&0.62004 \\
65&0.1535874&-0.209&0.1081632&-0.295&0.6897276&0.2226783&0.1568202&22&2.21214 \\
225&0.1219287&-0.186&0.0774765&-0.269&0.5157851&0.2363944&0.1502108&22&8.61654 \\
833&0.0969249&-0.175&0.0555005&-0.255&0.3942211&0.2458643&0.1407852&23&35.9982 \\
3201&0.0770270&-0.171&0.0396882&-0.249&0.3040212&0.2533606&0.1305442&23&144.185 \\
12545&0.0611994&-0.168&0.0283778&-0.246&0.2357796&0.2595619&0.1203573&24&608.702 \\
49665&0.0486160&-0.167&0.0203130&-0.243&0.1836408&0.2647342&0.1106127&24&2529.72 \\
197633&0.0386151&-0.167&0.0145686&-0.241&0.1435315&0.2690357&0.1015011&24&.11E+05 \\


==> ex35h4ini.tex <==
21&0.1711499&---&0.1293512&---&22&0.22401 \\
65&0.1308635&-0.238&0.0860870&-0.360&22&0.42403 \\
225&0.1039326&-0.186&0.0612225&-0.274&23&1.66810 \\
833&0.0826578&-0.175&0.0438478&-0.255&23&6.80443 \\
3201&0.0657091&-0.170&0.0314280&-0.247&23&27.2897 \\
12545&0.0522196&-0.168&0.0225589&-0.243&24&120.800 \\
49665&0.0414910&-0.167&0.0162319&-0.239&24&560.127 \\
197633&0.0329617&-0.167&0.0117169&-0.236&24&2678.24 \\

